Structured Reinforcement Learning for Media Streaming at the Wireless Edge

Media streaming is the dominant application over wireless edge (access) networks. The increasing softwarization of such networks has led to efforts at intelligent control, wherein application-specific actions may be dynamically taken to enhance the user experience. The goal of this work is to develop and demonstrate learning-based policies for optimal decision making to determine which clients to dynamically prioritize in a video streaming setting. We formulate the policy design question as a constrained Markov decision problem (CMDP), and observe that by using a Lagrangian relaxation we can decompose it into single-client problems. Further, the optimal policy takes a threshold form in the video buffer length, which enables us to design an efficient constrained reinforcement learning (CRL) algorithm to learn it. Specifically, we show that a natural policy gradient (NPG) based algorithm that is derived using the structure of our problem converges to the globally optimal policy. We then develop a simulation environment for training, and a real-world intelligent controller attached to a WiFi access point for evaluation. We empirically show that the structured learning approach enables fast learning. Furthermore, such a structured policy can be easily deployed due to low computational complexity, leading to policy execution taking only about 15$\mu$s. Using YouTube streaming experiments in a resource constrained scenario, we demonstrate that the CRL approach can increase quality of experience (QOE) by over 30\%.

==> GradientDominance.tex <==
\subsection{Convergence of NPG for Threshold Parameterization}
Consider the following primal dual method to solve the minimization problem ~\ref{eqn:CMDP}.
\begin{align}\label{eqn:pseudoNPGalgo}
\theta_{n,{t+1}}(s) &= \theta_{n,t}(s) - \eta_1 F_{\rho}(\theta_{n,t})^{\dagger} \nabla_{\theta_n}J^{\pi_{\theta_{n,t}}}(\rho_n;\lambda_t)\\
\lambda_{t+1} &= \cP_{\Lambda}(\lambda_t + \eta_2 \sum_{n=1}^N \nabla_{\lambda}J^{\pi_{\theta_{n,t}}}(\rho_n;\lambda_t)) \nonumber
\end{align}
where $\theta_{n,t}$ is the threshold parameter of client $n$ at time $t$, 
%$F_{\rho}(\theta_{n,t}) \triangleq \E_{(s,a)\sim \pi_{\theta_{n,t}}}[\nabla_{\theta_n} \log\pi_{\theta_{n,t}}(a|s) \nabla_{\theta_n} \log\pi_{\theta_{n,t}}(a|s)^\top]$ 
$F_{\rho}(\theta) \triangleq \E_{(s,a)\sim \pi_{\theta}}[\nabla_{\theta} \log\pi_{\theta}(a|s) (\nabla_{\theta} \log\pi_{\theta}(a|s))^\top]$ is the fisher information matrix induced by the policy $\pi_{\theta}$, $A^\dagger$ is the moore-penrose inverse of matrix $A$, and $\cP_{\Lambda}$ is the projection operator onto the interval $\Lambda$. $\eta_1$ and $\eta_2$ are constant step-sizes.

\textbf{Remarks:} Algorithm~\eqref{eqn:pseudoNPGalgo} is a straightforward extension of the standard primal dual approach to solve the saddle point problem~\eqref{eqn:saddlepoint}. The primal variables here are the threshold parameters of each client $n \in [N]$. At each iteration $t+1$, the threshold parameters of client $n$ follow an NPG update independent of the others. Intuitively, the update makes sense as it is known from Theorem~\eqref{eqn:decentpolthm}, it is sufficient to look at client policies which are independent of other but the respective value functions are coupled only through the dual variable $\lambda_t$ from the previous iteration $t$. The dual variable update at each iteration, however, uses the sum of gradients from each client $n$. It is easy to see that the our algorithm reduces to the standard primal dual method when $N=1$. 

We have the following provable guarantee for convergence of algorithm \eqref{eqn:pseudoNPGalgo}.
\begin{thm}\label{eqn:finiteconvthm}
For a given $\rho \triangleq \otimes_{i=1}^N \rho_n$, where $~\rho_n \in \triangle_{\cS_n}, \theta_{n,0}$ be the starting state distribution and threshold parameter initialization of client $n$, and $\lambda_0$ be the initial dual variable. For the particular choice of $\eta_1 = $, $\eta_2 = $, the iterates generated by the algorithm \eqref{eqn:pseudoNPGalgo} satisfy
\end{thm}
The proof technique we follow is similar to that of ~\cite{ding2020npg}. We first show that the NPG method has a simple parameter update for the threshold policy class. We then prove that the average cost function generated by the iterates of the algorithm converges to the global optimal value, and bound the constraint violation. The details are provided in Appendix~\ref{sec:convlogregobj}.
%\end{proof}



==> experiments/fig2dqsevoluation.tex <==
\begin{tikzpicture}
\begin{axis}[
    x label style={at={(axis description cs:0.5,0)},anchor=north},
    y label style={at={(axis description cs:0.12,.5)},anchor=south},
    xlabel={\footnotesize Time (in seconds)}, 
    ylabel={\footnotesize Quality of Experience}, 
    xmin=-3, xmax=78, ymin=1, ymax=5.5, line width=1pt,
    extra x ticks={10,30,50,70}]
        
        	\addplot[color=blue!50!black,dashed] coordinates {
		(1,1)
		(1,5)
		(22,5)
		(22,1)
	};
        	\addplot[color=blue!50!black,dashed] coordinates {
		(33,1)
		(33,5)
		(43,5)
		(43,1)
	};
	\addplot[color=blue!50!black,dashed] coordinates {
		(55,1)
		(55,5)
		(75,5)
	};
	\addplot[color=red!80!black,legend=test] coordinates {
	(1,5)
	(22,5)
	(27,3.2)
	(33,2.7)
	(36,4.3)
	(43,4.3)
	(45,4)
	(55,3.7)
	(75,3.8)
	};
\end{axis}

\begin{scope}[xshift=-2.8mm]
\node [draw, color=green!50!black, line width=0.8pt, single arrow,single arrow head extend=.3cm,rotate=45] at (1.8,4.45) {Stall};
\node [draw, color=green!50!black, line width=0.8pt, single arrow,single arrow head extend=.2cm,rotate=180] at (4.17,2.1) {\tikz\node[inner ysep = -3mm, inner xsep=1mm, rotate=180] {Play};};
\node [draw, color=green!50!black, line width=0.8pt, single arrow,single arrow head extend=.2cm,rotate=200] at (4.94,4.45) {\tikz\node[inner ysep = -3.5mm, inner xsep=-1mm, rotate=180] {Stall};};
\node [draw, color=green!50!black, line width=0.8pt, single arrow,single arrow head extend=.2cm,rotate=135] at (5.8,2.80) {\tikz\node[inner ysep = -3mm, inner xsep=1mm, rotate=180] {Play};};
\end{scope}

%legend
\begin{scope}[xshift=-8mm]
\draw[gray] (3.8,5.2) rectangle (6.75,5.5);
\draw[color=red!80!black, line width=1pt] (3.95,5.35) -- (4.5,5.35) ++(0.25,-0.01) node[color=black,scale=0.85] {\tiny\bf DQS};
\draw[color=blue!50!black,dashed, line width=1pt] (5.1,5.35) -- (5.6,5.35) ++(0.6,-0.01) node[color=black,scale=0.9] {\tiny\bf Play Status};
\end{scope}

\end{tikzpicture}

==> figures/fig2dqsevoluation.tex <==
\begin{tikzpicture}
\begin{axis}[
    x label style={at={(axis description cs:0.5,0)},anchor=north},
    y label style={at={(axis description cs:0.12,.5)},anchor=south},
    xlabel={\footnotesize Time (in seconds)}, 
    ylabel={\footnotesize Quality of Experience}, 
    xmin=-3, xmax=78, ymin=1, ymax=5.5, line width=1pt,
    extra x ticks={10,30,50,70}]
        
        	\addplot[color=blue!50!black,dashed] coordinates {
		(1,1)
		(1,5)
		(22,5)
		(22,1)
	};
        	\addplot[color=blue!50!black,dashed] coordinates {
		(33,1)
		(33,5)
		(43,5)
		(43,1)
	};
	\addplot[color=blue!50!black,dashed] coordinates {
		(55,1)
		(55,5)
		(75,5)
	};
	\addplot[color=red!80!black,legend=test] coordinates {
	(1,5)
	(22,5)
	(27,3.2)
	(33,2.7)
	(36,4.3)
	(43,4.3)
	(45,4)
	(55,3.7)
	(75,3.8)
	};
\end{axis}

\begin{scope}[xshift=-2.8mm]
\node [draw, color=green!50!black, line width=0.8pt, single arrow,single arrow head extend=.3cm,rotate=45] at (1.8,4.45) {Stall};
\node [draw, color=green!50!black, line width=0.8pt, single arrow,single arrow head extend=.2cm,rotate=180] at (4.17,2.1) {\tikz\node[inner ysep = -3mm, inner xsep=1mm, rotate=180] {Play};};
\node [draw, color=green!50!black, line width=0.8pt, single arrow,single arrow head extend=.2cm,rotate=200] at (4.94,4.45) {\tikz\node[inner ysep = -3.5mm, inner xsep=-1mm, rotate=180] {Stall};};
\node [draw, color=green!50!black, line width=0.8pt, single arrow,single arrow head extend=.2cm,rotate=135] at (5.8,2.80) {\tikz\node[inner ysep = -3mm, inner xsep=1mm, rotate=180] {Play};};
\end{scope}

%legend
\begin{scope}[xshift=-8mm]
\draw[gray] (3.8,5.2) rectangle (6.75,5.5);
\draw[color=red!80!black, line width=1pt] (3.95,5.35) -- (4.5,5.35) ++(0.25,-0.01) node[color=black,scale=0.85] {\tiny\bf DQS};
\draw[color=blue!50!black,dashed, line width=1pt] (5.1,5.35) -- (5.6,5.35) ++(0.6,-0.01) node[color=black,scale=0.9] {\tiny\bf Play Status};
\end{scope}

\end{tikzpicture}
